Modeling principles for a physiology-based whole-body model of human metabolism

Physiological whole-body models are valuable tools for the development of novel drugs where understanding the system aspects is important. This paper presents a generalized model that encapsulates the structure and flow of whole-body human physiology. The model contains vascular, interstitial, and cellular subcompartments for each organ. Scaling of volumes and blood flows is described to allow for investigation across populations or specific patient groups. The model equations and the corresponding parameters are presented along with a catalog of functions that can be used to define the organ transport model and the biochemical reaction model. A simple example illustrates the procedure.

==> tex/03data.tex <==
% puttet ind i methods. 
Blood flow volumes (Q) and organ volumes (V) for weights ranging from 70 to 110 kg and heights from 160 to 200 cm are presented for each compartment, derived from the integrated database in PKsim \cite{ICRPPub, PKsim}. Table XX displays the corresponding Q's and V's for the adipose compartment, while data from the remaining compartments can be found in Appendix X.

% adipose weight data here 
% adipose height data here 

==> tex/06conclusion.tex <==
\section{Conclusion}
% The model's framework is designed to facilitate the design, simulation, and exploration of therapeutic interventions within human physiology for drug discovery. It allows for customized drug response simulations, optimization of drug dosing regimens and can aid in identifying potential therapeutic targets. Integrating metabolic networks from various organ cells into the whole-body model becomes a key objective, enhancing research capabilities across a broader spectrum of human metabolic diseases and pushing the boundaries of pharmaceutical innovation.

% We presented a model structure and flow dynamics for the whole-body human physiology, and coupled this model to interstitial and cellular metabolic reactions. Furthermore, we presented a transport model and a biochemical model, and provided a catalog of reactions elements. We have placed a strong emphasis on the transparency of the underlying equations and ensured that the model is user-friendly, allowing for ease of use without the need for specialized software.   



==> tex/outline.tex <==
physiolgical whole-body flow model 

flow model 
diagram 
- vascular
- interstetium 
- intracellulær 

Generalized. Anatomisk/fysiologisk korrekt. 

PK-sim. 
skalering af volumes + blood flow rates. Tabeller. 

mand + kvinde. 

generalized ligninger 

+ minimal eksempel med rates. 


to do before wednesday: 
- figur wholebody (L)
- data afsnit med PKsim-data. (L)
    tabel/matrix med data (flere betydende cifre, 3 decimaler) for begge køn.   
    pointe: at PKsim genere personer med variabilitet. 
- plot med skalering 

minimal example. 

Diskussion: 
- det giver mening at det kun er muscle, adipose, skin..  



% volume
\begin{table}
\centering
\caption{Organ volumes in liter for a healthy European 30-year old male, with weight = 73 kg and height = 176 cm and a healthy European 30-year old female, with weight = 60 kg and height = 163 cm.}
\label{tab:Organ_volumes}
% \resizebox{\columnwidth}{!}
% {%
\begin{tabular}{lll}
\textbf{Organ}  & \multicolumn{2}{l}{\textbf{Value {[}L{]}}} \\ \hline
                & Male                & Female               \\ 
Arterial blood  & 0.419                & 0.320                 \\ % No
Venous blood    & 0.964                & 0.737                 \\ % No
Bone            & 11.819               & 9.122                 \\ % Yes
Brain           & 1.509                & 1.355                 \\ % Yes
Fat             & 14.652               & 19.420                \\ % Yes
Gonads          & 0.040                & 0.013                 \\ % Yes
Heart           & 0.417                & 0.329                 \\ % Yes
Kidney          & 0.438                & 0.404                 \\ % Yes
Large intestine & 0.413                & 0.417                 \\ % Yes
Liver           & 2.377                & 1.918                 \\ % Yes
Lung            & 1.215                & 0.946                 \\ % Yes
Muscle          & 32.645               & 20.288                \\ % Yes
Pancreas        & 0.190                & 0.170                 \\ % Yes
Portal Vein     & 1.037                & 0.793                 \\ % No
Saliva          & 0.006               & 0.00493              \\ % No
Skin            & 3.763                & 2.724                 \\ % Yes
Small intestine & 0.725                & 0.695                 \\ % Yes
Spleen          & 0.207                & 0.186                 \\ % Yes
Stomach         & 0.169                & 0.163                 \\ \hline % Yes
\end{tabular}%
% }
\end{table}
